Pricing Social Visibility Service in Online Social Networks: Modeling and Algorithms

Online social networks (OSNs) such as YoutTube, Instagram, Twitter, Facebook, etc., serve as important platforms for users to share their information or content to friends or followers. Oftentimes, users want to enhance their social visibility, as it can make their contents, i.e., opinions, videos, pictures, etc., attract attention from more users, which in turn may bring higher commercial benefit to them. Motivated by this, we propose a mechanism, where the OSN operator provides a "social visibility boosting service" to incentivize "transactions" between requesters (users who seek to enhance their social visibility via adding new "neighbors") and suppliers (users who are willing to be added as a new "neighbor" of any requester when certain "rewards" is provided). We design a posted pricing scheme for the OSN provider to charge the requesters who use such boosting service, and reward the suppliers who contribute to such boosting service. The OSN operator keeps a fraction of the payment from requesters and distributes the remaining part to participating suppliers "fairly" via the Shapley value. The objective of the OSN provider is to select the price and supplier set to maximize the total amount of revenue under the budget constraint of requesters. We first show that the revenue maximization problem is not simpler than an NP-hard problem. We then decomposed it into two sub-routines, where one focuses on selecting the optimal set of suppliers, and the other one focuses on selecting the optimal price. We prove the hardness of each sub-routine, and eventually design a computationally efficient approximation algorithm to solve the revenue maximization problem with provable theoretical guarantee on the revenue gap. We conduct extensive experiments on four public datasets to validate the superior performance of our proposed algorithms.

==> 4_division_shiyuan.tex <==
% !TEX root = main-Hong.tex

\section{\bf Algorithm for Fair Division of Contribution}

%To incentivize suppliers to participate, 
%one needs to divide $q R (p,q, \mathcal{M})$ fairly among suppliers. 
We use the idea of Shapley values to split the reward fairly
among participating suppliers, 
which prescribes a contribution denoted by $\phi_u (p, \mathcal{M})$ 
for each participating supplier.  
Such mechanism can make sure that 
a supplier is willing to participant in the social visibility boosting service 
if his per unit valuation does not exceed the per unit price 
that the OSN operator pays, i.e., $q_u \leq q$.  


\noindent
{\bf The Shapley value.}
The Shapley value is a cornerstone in cooperative game theory 
and it aims to fairly divide the pay off among a set of players. 
For Problem~\ref{prob},
the selected set of suppliers  $\mathcal{M}^\ast$ of size $b$
can be regarded as the coalition in the cooperatives game, 
each supplier $u \in \mathcal{M}^\ast$ can be regarded as an individual player.
Let $\nu( \mathcal{M})=q I(p, \mathcal{M}^\ast)$ be the characteristic function.
The Shapley value of each individual supplier $u \in \mathcal{M}^\ast$ can be computed as follows: 
\begin{align}
	\label{eq:shapley}
	\phi_u (p, \mathcal{M}^\ast) 
	= \sum_{\mathcal{S}\subset {\mathcal{M}} \setminus\{u\}  }  
	\frac{|\mathcal{S}|!(b-|\mathcal{S}|-1)!}{b!} (  \nu( \mathcal{S}\cup \{u\})  - \nu(\mathcal{S}) ). 
\end{align}

The cost of a participating supplier  $u$ is defined as
\[
c_u(p, \mathcal{M}^\ast) = \nu(\{u\}) = q_u I(p, \mathcal{M}^\ast) . 
\] 

We have the following theorem about the willingness of user $u \in \mathcal{U}$  
to participate in the  social visibility boosting service.
\begin{thm}
	If a supplier $u \in \mathcal{U}$ has  $q_u \geq  \alpha p $, 
	then $u$ would be unwilling to join $\mathcal{U}$, i.e., $u \in \widetilde{R}(p)$.
\end{thm}
\noindent
\textbf{Proof.}
The characteristic function is submodular thus subadditive, i.e., 
\[
\nu( \mathcal{M}_1 \sqcup \mathcal{M}_2) \leq \nu(\mathcal{M}_1) + \nu(\mathcal{M}_2).
\] 
According to the \textit{stand-alone test} property of Shapley value, we have
% TODO 加这个property的ref
%$$\phi_l \leq \alpha p  f(\{l\}). $$
\[
\phi_u (p, \mathcal{M}^\ast)  \leq \nu(\{u\}). 
\]
Since $q_u \geq \alpha p $, we have
\[
\nu(\{v\}) = \alpha p I(p, \{u\})  \leq q_u I(p, \{u\}). 
\] 
Thus, we have have
\[ 
\phi_u (p, \mathcal{M}^\ast) \leq  q_u I(p, \{u\}) = c_u(p, \mathcal{M}^\ast). 
\]  
It shows that, 
for user $u \in \mathcal{R}$ whose unit valuation $q_u \geq \alpha p$, 
the reward received by Shapley value based dividing rule can not be greater than the cost,
thus he is not willing to participant in the social visibility boosting service.



\begin{asum} 
	%[Risk preference.]
	We assume that 
	if a supplier $u \in \mathcal{R}$ has $q_u \leq \alpha p$,
	then $u$ would be willing to participant in the social visibility boosting service,
	i.e., $u \in \widetilde{R}(p)$
	\label{asum:willing}
\end{asum}
Assumption~\ref{asum:willing} indicates that, 
only if there is a chance to satisfy
\[ 
\phi_u (p, \mathcal{M}^\ast) \geq   c_u(p, \mathcal{M}^\ast),
\]  
then the user would be willing to take the risk. % to get the surplus.

\noindent
{\bf Algorithm to compute the Shapley value. }  
Indeed, 
using the original Shapley value formula involves computing 
the marginal contribution of every player 
to every coalition has an exponential complexity. 
So it is clearly prohibitive for bigger scale (of, e.g, 100 or 1000 players). 
Therefore, the specific challenge we tackle is to efficiently compute the Shapley value. 


Denote an ordering of the players as 
$\sigma = (u_1,\cdots,u_b)$,
where $u_i \in \mathcal{M}^\ast$ denotes the player in the $i-$th order.
Denote the set of players ranked before player $i$ in the order $\sigma$ as
\begin{equation}
	\mathcal{S}_i^\sigma \triangleq \{ \text{all players ranked before } u_i \text{ in the order } \sigma \}.
	\label{eq:shapley1}
\end{equation}
Shapley value expressed in Equation~\eqref{eq:shapley} can be rewritten as 
\begin{equation}
	\hat{\phi}_{u_i} = \mathbb{E}[\Delta(\sigma , u_i) ].
	\label{eq:shapley2}
\end{equation}
where  $\Delta(\sigma , u_i)$ is defined as 
\begin{equation}
	\Delta(\sigma,u_i) 
	\triangleq 
	\nu(\mathcal{S}_i^\sigma \cup \{u_i\}) - \nu(\mathcal{S}_i^\sigma ).
\end{equation}

Algorithm~\ref{algo:shapley} outlines a Monte Carlo algorithm 
to approximate the Shapley value of each participating supplier.

\begin{algorithm}[H] 
	\begin{algorithmic}[1]
		\STATE \textbf{input:} coalition $ \mathcal{L}$, sample size $K$, link $l$
		\STATE \textbf{output:} $\hat{\phi}_{u}$
		%		\STATE init $\mathcal{L}=\emptyset, \mathcal{S} = \mathcal{U} \times \mathcal{R}$
		\FOR{$k=1$ to $K$}
		\STATE generate a ordering $\sigma$ using Monte Carlo Sampling
		\STATE   $\hat{\phi}_{u} \leftarrow \frac{(k-1)\hat{\phi}_{u} + \nu(\mathcal{S}_i^\sigma \cup \{u\}) - \nu(\mathcal{S}_i^\sigma ) }{k} $
		\ENDFOR
		\RETURN average($\hat{\phi}_{u}$)
	\end{algorithmic}
	\caption{Sampling based Shapley value algorithm}
	\label{algo:shapley}
\end{algorithm}




%\begin{thm} 
%	
%	The output $\hat{\phi}_{\sigma_n}$ of Algorithm~\ref{algo:shapley} satisfies
%	\begin{align*}
%	| \hat{\phi}_{\sigma_n}- \phi_{\sigma_n} | 
%	\leq \frac{\max_{\sigma \in \Omega} \Delta(\sigma , {\sigma_n}) - \min_{\sigma \in \Omega} \Delta(\sigma , {\sigma_n}) }{\sqrt{K}}  
%	\sqrt{\frac{1}{2} \ln \frac{2}{\delta} },
%	\end{align*}
%	with a probability of at least $1-\delta$, where $\delta \in (0,1]$ 
%	and $\Omega$ is the sample space with $|\Omega|=b!$.
%\end{thm}

